NeuronEye: Query-Guided Visual Concept Activation for Vision-Language Reasoning

Current vision-language models (VLMs) encode visual information in dense hidden states where object identity, spatial layout, and local attributes are implicitly entangled rather than explicitly disentangled, limiting their ability to isolate and modulate the specific visual evidence required by a given language query. Inspired by sparse population coding and top-down modulation in biological vision, we introduce NeuronEye, a plug-in framework that constructs a sparse, concept-level neuron vocabulary from intermediate VLM representations and selectively activates query-relevant visual concepts during inference. NeuronEye decomposes vision-token states into an overcomplete sparse basis organized by concept-level clusters, uses the language query to activate relevant clusters and localize the patches where selected concepts are expressed, and injects the focused evidence back into vision tokens. A complementary suppression mechanism attenuates dominant perceptual directions to preserve weaker but relevant cues. All operations run in a single forward pass over a frozen VLM backbone. On Qwen2.5-VL-7B, NeuronEye raises CV-Bench overall accuracy by +3.1 with gains of +9.5 on Distance, and improves BLINK Multi-view by +8.3, with similar trends on LLaVA-1.6-7B. These results suggest that sparse neuron vocabularies can serve not only as post-hoc interpretability tools but also as active interfaces for concept-level visual reasoning.

==> backup.tex <==
% Current vision-language models (VLMs) extract visual features once through an image encoder and pass them, unchanged, to a language model---the visual representation remains static throughout inference regardless of the query. We introduce NeuronEye, a framework that transforms sparse neuron space from a passive interpretability lens into an active computational substrate for inference-time visual reasoning. NeuronEye comprises three components. \emph{Sparse Neuron Space} (SNS) projects dense visual representations into an overcomplete sparse basis via a frozen sparse autoencoder and organizes the resulting neurons into semantically coherent clusters. \emph{Neuron-guided Visual Focus} (NVF) performs query-conditioned reasoning by routing language queries to task-relevant neuron clusters, refining selected sparse features through a semantic completion module, and injecting the completed representations back into vision tokens via localized cross-attention. \emph{Perceptual Concept Suppression} (PCS) counteracts the representational anisotropy amplified by focus-driven modulation, suppressing dominant spectral directions to preserve feature diversity.

% The primate visual cortex does not process scenes through dense, undifferentiated activation. Instead, it employs sparse, selective firing: only a small fraction of neurons are active at any moment, each tuned to specific visual concepts---edges in V1~\cite{olshausen1996emergence}, object parts in V4~\cite{desimone1984stimulus}, faces and categories in the inferotemporal cortex~\cite{quiroga2005invariant,rolls1995sparseness}. Crucially, this sparse code is not merely an efficient encoding scheme~\cite{barlow1972single}; it enables flexible cognition by allowing top-down attention to selectively gate individual features in response to behavioral demands~\cite{desimone1995neural}. The decomposability of the code is what makes the computation adaptive.

% Current VLMs extract visual features once through an image encoder and pass them, unchanged, to a language model~\cite{liu2023visual, bai2024qwenvl, qwen2.5vl, li2024llavaonevision}. The language side iterates across dozens of transformer layers, progressively refining what to say; the visual side is frozen after a single forward pass, with no mechanism to revisit or restructure what to see. When this static representation proves insufficient---as it often does for spatial reasoning, compositional understanding, or multi-view tasks---practitioners compensate through external scaffolding: retrieval pipelines~\cite{zelikman2022star}, tool calls~\cite{yao2023react}, and multi-agent orchestration~\cite{park2023generative}. These approaches improve performance by extending the system beyond a single forward pass, but they shift the locus of reasoning from the model's internal computation to system-level orchestration. The underlying visual representation remains untouched.

% We take a different path. Rather than augmenting the system externally, we ask whether the model's own representations can be restructured into a form that supports dynamic, query-conditioned computation. This requires a representational medium with three properties: \emph{decomposability} into individually meaningful units that can be independently addressed, \emph{selectivity} that allows activating or suppressing features conditioned on the current reasoning state, and \emph{stability} under iterative manipulation to avoid representational collapse. Dense, entangled embeddings satisfy none of these. Recent work on sparse autoencoders (SAEs)~\cite{bricken2023monosemanticity} has shown that model activations can be decomposed into monosemantic features, achieving the first property. Yet SAEs remain tools for post-hoc interpretation and ad-hoc feature steering---they do not participate in inference dynamics, and the second and third properties are entirely unaddressed.

% This paper introduces NeuronEye, a framework that transforms sparse neuron space from a passive interpretability lens into an active computational substrate for inference-time visual reasoning. NeuronEye comprises three components, each targeting one of the above properties. First, we construct a \emph{Sparse Neuron Space} (SNS) by projecting visual representations into a high-dimensional sparse basis and organizing the resulting neurons into semantically coherent clusters, yielding a compositional feature vocabulary (\emph{decomposability}). Second, \emph{Neuron-guided Visual Focus} (NVF) performs query-conditioned selection and transformation within this space: a lightweight router activates task-relevant neuron clusters based on the language query, and a semantic completion module injects refined features into localized image patches via cross-attention (\emph{selectivity}). Third, \emph{Perceptual Concept Suppression} (PCS) counteracts the anisotropy amplified by focus-driven modulation, suppressing dominant spectral directions to preserve feature diversity (\emph{stability}). Together, these mechanisms form a unified computational loop that enables the model to reason \emph{through} its representations, not merely over them.

% \paragraph{External augmentation for VLM reasoning.}
% A growing body of work improves VLM reasoning through system-level augmentation: tool use~\cite{yao2023react}, retrieval-augmented generation~\cite{zelikman2022star}, chain-of-thought prompting~\cite{wei2022chain}, and multi-agent pipelines~\cite{park2023generative}. These approaches decompose complex problems and delegate sub-tasks to external modules, effectively extending the model beyond a single forward pass. While effective, they shift the locus of reasoning from internal computation to orchestration, introducing latency, error propagation, and pipeline complexity. More fundamentally, the visual representation consumed by the model remains static throughout---external modules compensate for, rather than resolve, the inability of the model to dynamically restructure its own features. NeuronEye is orthogonal to these methods: rather than adding external modules, NVF restructures the visual representation \emph{within} the model's own forward pass by routing queries to task-relevant neuron clusters and injecting refined features directly into vision tokens. The two paradigms are complementary and can in principle be combined.

% Modern vision-language models (VLMs) align image and text by jointly processing visual and language tokens through attention-based multimodal fusion~\cite{liu2023visual,bai2024qwenvl,qwen2.5vl,li2024llavaonevision}. Although effective, this alignment occurs in dense hidden space, where each visual token may entangle object identity, spatial layout, local attributes, and background context. This makes it difficult to isolate the evidence needed for spatial, relational, or localization-sensitive reasoning.

% Biological vision offers a useful intuition: visual processing is sparse and selective, with only a subset of neurons responding strongly to particular visual patterns. Inspired by this principle, we ask whether intermediate VLM representations can be organized into sparse, addressable visual features that can be selected and modulated according to a language query.

% Existing methods only partially address this goal. Vision-token selection or reduction methods retain, merge, or discard visual tokens, but still treat each selected patch as a dense unit. Representation-level steering methods modify hidden states more directly, but are often global and not explicitly tied to query-conditioned visual concepts. Moreover, focused modulation can overemphasize a few high-energy perceptual directions, suppressing weaker but relevant cues. This motivates a mechanism that selects query-relevant sparse visual features while rebalancing the resulting representation.

% We introduce \emph{NeuronEye}, a framework for query-guided visual reasoning through sparse neuron-level features. NeuronEye first constructs a \emph{Sparse Neuron Space} (SNS), which projects intermediate vision-token states into an overcomplete sparse basis using a sparse autoencoder and groups sparse neurons into concept-level clusters. These clusters serve as routing targets for \emph{Neuron-guided Visual Focus} (NVF): given a language query, NVF predicts relevant neuron-cluster indices, uses a vision-side scorer to encourage image-supported selection, modulates the SAE latent dimensions within selected clusters, and injects the decoded features back into localized vision tokens through cross-attention. Since this focused modulation can concentrate the representation along dominant perceptual directions, \emph{Perceptual Concept Suppression} (PCS) attenuates these directions at a later layer to preserve weaker visual cues.

% NeuronEye is a targeted sparse feature-level alignment mechanism rather than a general-purpose reasoning enhancer. During inference, all operations run within a single forward pass; the VLM backbone and SAE remain frozen, and no external annotator, retrieval system, tool use, or multi-pass decoding is used.

% Our contributions are threefold:
% (1) we introduce a shift from interpreting SAE neurons after the fact to using them as an inference-time control interface for VLM visual reasoning, by decomposing intermediate vision-token states into addressable sparse features and organizing them into concept-level neuron clusters. (2) we develop a feature-level intervention pipeline that treats sparse neuron clusters as a query-conditioned routing interface, where NVF selects and injects localized visual evidence based on query intent and image evidence, while PCS mitigates over-concentration after focused modulation.
% and (3) we evaluate NeuronEye across spatial, multi-view, localization, and open-ended VQA benchmarks, demonstrating consistent gains on structure-sensitive tasks as well as clear limitations under domain shift. Experiments on CV-Bench, BLINK, RealWorldQA, and MMStar show that NeuronEye improves Qwen2.5-VL-7B across benchmarks, with especially large gains on CV-Bench Distance (+9.5) and BLINK Multi-view (+8.3). Ablations show that each component plays an important role in the final performance.


% \paragraph{Sparse autoencoders and mechanistic interpretability.}
% Sparse autoencoders (SAEs) decompose superposed activations into sparse and more interpretable latent features~\cite{cunningham2024sparse, wang2025sparse}. Existing work mainly uses SAE features for interpretability, by identifying human-understandable directions in model representations, or for steering, by activating or suppressing selected latent directions to bias model outputs toward certain content~\cite{zou2024representation, rimsky2024steering}. NeuronEye extends the use of SAE features from post-hoc analysis and steering to inference-time visual reasoning. It organizes SAE-derived visual features into neuron clusters, i.e., groups of sparse features associated with related visual concepts, and treats these clusters as index-level routing units for downstream reasoning.

% \paragraph{Implicit and explicit visual-language alignment.}
% When SAE-derived features are used for VLM reasoning, the key question becomes how a language query should select the visual evidence needed for an answer. Modern VLMs align image and text by jointly processing visual and language tokens through self-attention or cross-attention, but this fusion occurs in dense hidden space, where each visual token may entangle object identity, spatial layout, texture, and background context. In VQA, this becomes a bottleneck when the answer depends on localized evidence, such as whether a person is holding an object, whether two objects are spatially related, or whether all instances share an attribute. Prior work explores explicit grounding through attention maps, region selection, or visual-token pruning, but these methods usually operate over dense tokens or image regions. NeuronEye instead links query-conditioned routing to structured neuron clusters, allowing visual evidence to be selected at the sparse feature level rather than only at the patch-token level.

% \paragraph{Visual attention and representation adaptation.}
% Attention mechanisms, visual grounding, and cross-modal alignment allow VLMs to associate queries with relevant image regions~\cite{radford2021learning, liu2023visual, bai2024qwenvl}. However, these methods operate within a largely static, feed-forward paradigm: visual features are reweighted but not fundamentally transformed, and the representation basis remains fixed after encoding. Iterative refinement approaches~\cite{banino2021pondernet, darcet2024vision} and feature denoising methods adjust importance weights but do not restructure the underlying feature space. This limitation is compounded by the anisotropy of transformer representations~\cite{ethayarajh2019anisotropy}, where information concentrates along a small number of dominant directions, reducing effective feature diversity. Existing solutions primarily address this issue at training time through regularization or architectural modifications, offering limited flexibility at inference time. NeuronEye targets this gap at two levels: NVF operates in a sparse, overcomplete basis rather than the original dense embedding space, enabling localized feature injection that goes beyond reweighting; PCS then counteracts the anisotropy amplified by this injection by suppressing dominant spectral directions at a later layer, preserving the geometric diversity that standard attention mechanisms leave unprotected.

% \paragraph{Visual-token reduction and feature-level adaptation.}
% This feature-level view distinguishes NeuronEye from methods that modify visual processing at the token or dense-representation level. Token-reduction methods, such as FastV and SparseVLM, improve efficiency by removing, merging, or retaining visual tokens, while representation-level intervention methods, such as SAVE and VISTA, steer dense hidden states to enhance visual information or reduce hallucination. In contrast, NeuronEye targets a different abstraction level: it intervenes on sparse visual features within localized regions, refining evidence without discarding tokens or applying a global dense-state shift.


% Vision-token reduction methods~\cite{chen2024fastv,zhang2025sparsevlm} prune or merge patches but leave each retained token dense. Representation-level interventions~\cite{park2025save,li2025vista} steer global hidden states without conditioning on which visual concept a query demands. The core difficulty remains: dense visual representations lack a mechanism for isolating and selectively modulating individual visual concepts according to the question at hand.




\section{Experiments}

The SAE is trained on vision-token activations from the full VQAv2 training set and frozen for all subsequent stages.

\subsection{Implementation and Data Setup}
\label{sec:exp_setup}

\paragraph{Model setup.}
We use Qwen2.5-VL-7B as the frozen base model. NeuronEye constructs the SNS at layer $\ell=8$ and groups its sparse features into $K=64$ neuron clusters. The VLM backbone, SNS, and neuron-cluster assignments remain frozen in all subsequent experiments. Based on this fixed SNS, NVF is applied at layer $\ell=8$, and PCS is applied at a later layer $\ell'=20$. The lightweight reasoning modules are fine-tuned using the two-stage procedure described in Appendix~\ref{app:training_hyperparams}, where we also report the full hyperparameter settings. All experiments are conducted on NVIDIA RTX PRO 6000 GPUs.

\paragraph{Data setup.}
All training data are independent of the evaluation benchmarks. VQAv2~\cite{antol2015vqa} is used only for SNS construction and lightweight module training: SNS is built from vision-token hidden states extracted over the full VQAv2 training set, while the lightweight reasoning modules are fine-tuned on randomly sampled 5K VQA subsets. For each subset, we assign cluster-index labels to supervise the NVF cluster predictor. These labels contain only index information; cluster descriptions are not used as textual evidence. We construct three independent supervision sets, train NeuronEye separately on each, and report the mean and standard deviation across the three runs.



\subsection{Evaluation Protocol}
\label{sec:evaluation}

We evaluate NeuronEye on vision-centric reasoning benchmarks covering spatial understanding, counting, relational perception, localization, and real-world visual reasoning. CV-Bench~\cite{tong2024cvbench} is our primary benchmark, with Count, Depth, Distance, and Relation sub-tasks directly testing structured visual understanding. We also evaluate on BLINK~\cite{fu2024blink} for multi-view reasoning and localization, and on RealWorldQA~\cite{xai2024realworldqa} and MMStar~\cite{chen2024mmstar} for broader visual question answering. CV-Bench, BLINK, RealWorldQA, and MMStar are used only for evaluation and are not used for SAE training or module fine-tuning. All evaluations use greedy decoding with temperature $0$ and no sampling, ensuring deterministic outputs.



==> checklist.tex <==
\section*{NeurIPS Paper Checklist}




\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction describe NeuronEye as an inference-time reasoning framework that operates through sparse neuron representations for visual understanding. The claims are supported by the reported experiments, ablations, and limitations, and the scope is restricted to vision-language reasoning tasks evaluated in this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper includes a dedicated limitations discussion. It states that the method depends on the coverage of the learned SNS neuron vocabulary, the quality of neuron clustering and routing supervision, and the general-domain nature of the VQAv2-trained sparse vocabulary. It also reports domain-shift degradation and inference/memory overhead.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not present formal theoretical theorems or proof-based claims. The contribution is methodological and empirical.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper describes the base model, SNS construction, training data, evaluation benchmarks, ablation settings, decoding strategy, and implementation details necessary to reproduce the main results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments are based on publicly available datasets and open-source base models. The full implementation, including the code repository, configuration files, data preparation instructions, and evaluation scripts, will be made publicly available upon acceptance to support reproduction of the main experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimental section reports the base VLM, plug-in layer, sparse latent configuration, neuron clustering setting, fine-tuning subset, trainable modules, evaluation datasets, decoding setup, and ablation variants. Additional implementation details are provided in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper reports mean and standard deviation across repeated runs in which the lightweight NeuronEye modules are trained on different randomly sampled 5K fine-tuning subsets. We specify this source of variation and use the same evaluation protocol, benchmark splits, and decoding strategy for the base model, NeuronEye, and all ablation variants.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper reports the GPU setup used for training and evaluation, along with latency, memory overhead, and parameter footprint comparisons between the base model and NeuronEye variants.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The work uses publicly available datasets and models for visual reasoning evaluation and does not involve private data collection, human-subject experiments, or deceptive deployment. The experiments are conducted for research purposes and follow standard responsible ML practice.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses that sparse neuron reasoning may improve interpretability and reliability of vision-language models, while also noting that stronger visual reasoning systems may inherit risks from the underlying VLMs, including hallucination, bias, and misuse in high-stakes settings.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release a new pre-trained foundation model, image generator, or scraped dataset with high misuse risk. The method builds lightweight reasoning modules on top of existing VLMs and uses standard public benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper properly credits the datasets, benchmarks, and model checkpoints used in the experiments through citations to their original papers or public release pages. All assets are publicly available resources and are used only for training or evaluation. The released code will provide instructions for obtaining each asset from its official source and will preserve the corresponding license and terms-of-use information.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not introduce a new dataset or benchmark. The learned modules and implementation are methodological artifacts rather than a new standalone dataset asset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing experiments or human-subject data collection.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve human-subject research, participant recruitment, or private human data collection.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper uses a vision-language model as the base model and, where applicable, uses a VLM-based annotator to assign semantic descriptions to top-activating SNS features. These uses are part of the methodological pipeline and are described in the method and implementation sections.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}
